FLIP: Towards Comprehensive and Reliable Evaluation of Federated Prompt Learning

The increasing emphasis on privacy and data security has driven the adoption of federated learning, a decentralized approach to train machine learning models without sharing raw data. Prompt learning, which fine-tunes prompt embeddings of pretrained models, offers significant advantages in federated settings by reducing computational costs and communication overheads while leveraging the strong performance and generalization capabilities of vision-language models such as CLIP. This paper addresses the intersection of federated learning and prompt learning, particularly for vision-language models. In this work, we introduce a comprehensive framework, named FLIP, to evaluate federated prompt learning algorithms. FLIP assesses the performance of 8 state-of-the-art federated prompt learning methods across 4 federated learning protocols and 12 open datasets, considering 6 distinct evaluation scenarios. Our findings demonstrate that prompt learning maintains strong generalization performance in both in-distribution and out-of-distribution settings with minimal resource consumption. This work highlights the effectiveness of federated prompt learning in environments characterized by data scarcity, unseen classes, and cross-domain distributional shifts. We open-source the code for all implemented algorithms in FLIP to facilitate further research in this domain.

==> acknowledgements.tex <==
\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2024/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to automatically hide this section in the anonymized submission.
\end{ack}


==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{This paper
    presents a federated prompt learning benchmark,
    \name{},
    to evaluate the performance
    of federated prompt learning algorithms
    in scenarios characterized by data scarcity,
    unseen classes, and cross-domain distributional shifts.
    We provide a comprehensive benchmark
    to evaluate the performance of federated prompt learning baselines
    and a set of evaluation metrics
    to assess the performance of these algorithms.}
  \item Did you describe the limitations of your work?
    \answerYes{Please refer to \Cref{app:discussion:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Please refer to \Cref{app:discussion:impact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{This paper does not include theoretical results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{This paper does not include theoretical results.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The codebase and instructions
    are available at \url{https://github.com/0-ml/flip}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please refer to \Cref{app:setup}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report error bars in result tables.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please refer to \Cref{app:discussion:resources}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{All datasets and models used in this work are cited.}
  \item Did you mention the license of the assets?
    \answerYes{Please refer to the codebase for the license information.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{All new assets are included in the codebase.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All datasets used in our work are publicly available.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{This paper does not use any personal data.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{This paper does not involve human subjects.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{This paper does not involve human subjects.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{This paper does not involve human subjects.}
\end{enumerate}

\end{enumerate}


==> tables/base2novel.tex <==
\begin{table}[t]
    \centering
    \caption{%
        \textbf{Comparison of novel class accuracy
        \textaccnovel{} (\%)
        of federated prompt learning methods.}
        Results are reported
        in similar style as \Cref{tab:global}.
        Note that ``\textaccbase{}'', ``\textaccnovel''
        and ``\textaccharmonic{}'' rows
        correspond to base \textaccbase{}
        and novel class \textaccnovel{} accuracies,
        and their harmonic mean
        \( \accharmonic \triangleq 2 / (\accbase^{-1} + \accnovel^{-1}) \),
        respectively.
        Only \textaccharmonic{} rows
        are used to rank best and second-best results,
        gray rows do not participate in ranking.
    }\label{tab:novel}
    % \setstretch{0.8}
    \adjustbox{max width=\linewidth}{%
    \begin{tabular}{lc|rrrr|r|c}
        \toprule
        \theader{} % Base \& Novel}
            & \multicolumn{1}{c|}{\hspace{-20pt}Metric}
            & \theader{Caltech} & \theader{Aircraft}
            & \theader{Cars} & \theader{Flowers}
            & \multicolumn{1}{|c|}{\textbf{Avg.}} & \theader{\#} \\
        \midrule
        \textbf{CLIP-ZS}
            &
            & 72.3 & 14.4
            & 41.8 & 56.6
            & 46.3 & 0 \\
        \midrule
        \multirow[c]{3}{*}{\textbf{PromptFL}}
            & \textaccbase{}
            & \tgpm{84.4}{0.8} & \tgpm{20.0}{0.5}
            & \tgpm{51.5}{0.5} & \tgpm{76.6}{1.9}
            & \textcolor{gray}{58.1} & \textcolor{gray}{--} \\
            & \textaccnovel{}
            & \tgpm{72.8}{1.1} & \tgpm{22.0}{0.6}
            & \tgpm{53.3}{0.3} & \tgpm{60.5}{1.4}
            & \textcolor{gray}{52.1} & \textcolor{gray}{--} \\
            & \textaccharmonic{}
            & \tpm{78.2}{1.0} & \tpm{20.9}{0.4}
            & \tpm{52.4}{0.3} & \tpm{67.6}{1.3}
            & 54.8 & 0 \\
        \midrule
        \multirow[c]{3}{*}{\textbf{FedOTP}}
            & \textaccbase{}
            & \tgpm{84.8}{0.4} & \tgpm{20.1}{0.2}
            & \tgpm{51.1}{0.3} & \tgpm{82.8}{3.1}
            & \textcolor{gray}{59.7} & \textcolor{gray}{--} \\
            & \textaccnovel{}
            & \tgpm{72.7}{0.5} & \tgpm{22.3}{0.9}
            & \tgpm{52.4}{0.7} & \tgpm{56.3}{0.2}
            & \textcolor{gray}{50.9} & \textcolor{gray}{--} \\
            & \textaccharmonic{}
            & \tpm{78.3}{0.4} & \tbpm{21.2}{0.3}
            & \tpm{51.7}{0.4} & \tpm{67.0}{1.0}
            & 54.5 & 2 \\
        \midrule
        \multirow[c]{3}{*}{\textbf{\fed{CoCoOp}}}
            & \textaccbase{}
            & \tgpm{79.9}{0.6} & \tgpm{14.4}{2.9}
            & \tgpm{48.7}{0.8} & \tgpm{74.6}{0.6}
            & \textcolor{gray}{54.4} & \textcolor{gray}{--} \\
            & \textaccnovel{}
            & \tgpm{71.6}{2.2} & \tgpm{13.6}{7.0}
            & \tgpm{52.2}{0.9} & \tgpm{56.1}{1.9}
            & \textcolor{gray}{48.4} & \textcolor{gray}{--} \\
            & \textaccharmonic{}
            & \tpm{75.5}{1.2} & \tpm{13.5}{5.6}
            & \tpm{50.4}{0.8} & \tpm{64.0}{1.0}
            & 50.8 & 0 \\
        \midrule
        \multirow[c]{3}{*}{\textbf{\fed{PLOT}}}
            & \textaccbase{}
            & \tgpm{84.5}{0.5} & \tgpm{20.5}{1.1}
            & \tgpm{51.0}{0.6} & \tgpm{80.7}{4.5}
            & \textcolor{gray}{59.1} & \textcolor{gray}{--} \\
            & \textaccnovel{}
            & \tgpm{73.4}{1.4} & \tgpm{21.4}{1.1}
            & \tgpm{51.4}{0.8} & \tgpm{57.3}{2.6}
            & \textcolor{gray}{50.8} & \textcolor{gray}{--} \\
            & \textaccharmonic{}
            & \tbpm{78.6}{1.0} & \tpm{20.9}{0.9}
            & \tpm{51.2}{0.5} & \tpm{66.9}{1.8}
            & 54.4 & 2 \\
        \midrule
        \multirow[c]{3}{*}{\textbf{\fed{ProDA}}}
            & \textaccbase{}
            & \tgpm{83.7}{1.1} & \tgpm{19.4}{0.7}
            & \tgpm{51.5}{0.9} & \tgpm{82.4}{3.3}
            & \textcolor{gray}{59.3} & \textcolor{gray}{--} \\
            & \textaccnovel{}
            & \tgpm{72.6}{1.1} & \tgpm{20.7}{1.1}
            & \tgpm{53.5}{0.8} & \tgpm{58.1}{2.1}
            & \textcolor{gray}{51.2} & \textcolor{gray}{--} \\
            & \textaccharmonic{}
            & \tpm{77.7}{0.4} & \tpm{20.0}{0.9}
            & \tbpm{52.5}{0.5} & \tpm{68.0}{1.0}
            & 54.6 & 2 \\
        \midrule
        \multirow[c]{3}{*}{\textbf{\fed{ProGrad}}}
            & \textaccbase{}
            & \tgpm{84.0}{0.2} & \tgpm{20.3}{0.8}
            & \tgpm{51.2}{0.7} & \tgpm{79.9}{1.0}
            & \textcolor{gray}{58.9} & \textcolor{gray}{--} \\
            & \textaccnovel{}
            & \tgpm{73.5}{0.8} & \tgpm{22.2}{1.7}
            & \tgpm{53.8}{0.3} & \tgpm{60.5}{1.5}
            & \textcolor{gray}{52.5} & \textcolor{gray}{--} \\
            & \textaccharmonic{}
            & \tupm{78.4}{0.5} & \tbpm{21.2}{1.2}
            & \tpm{52.5}{0.4} & \tpm{68.8}{0.6}
            & \textbf{55.2} & \textbf{4} \\
        \midrule
        \multirow[c]{3}{*}{\textbf{\fed{SRC}}}
            & \textaccbase{}
            & \tgpm{84.6}{0.8} & \tgpm{20.0}{1.1}
            & \tgpm{51.2}{0.4} & \tgpm{81.5}{0.8}
            & \textcolor{gray}{59.3} & \textcolor{gray}{--} \\
            & \textaccnovel{}
            & \tgpm{73.0}{1.1} & \tgpm{21.9}{1.6}
            & \tgpm{53.4}{0.5} & \tgpm{60.4}{1.6}
            & \textcolor{gray}{52.2} & \textcolor{gray}{--} \\
            & \textaccharmonic{}
            & \tupm{78.4}{0.3} & \tpm{20.8}{0.5}
            & \tpm{52.3}{0.2} & \tbpm{69.3}{1.1}
            & \underline{55.2} & 2 \\
        \midrule
        \multirow[c]{3}{*}{\textbf{\fed{KgCoOp}}}
            & \textaccbase{}
            & \tgpm{84.4}{0.5} & \tgpm{19.8}{0.3}
            & \tgpm{51.8}{1.0} & \tgpm{81.7}{2.8}
            & \textcolor{gray}{59.4} & \textcolor{gray}{--} \\
            & \textaccnovel{}
            & \tgpm{73.2}{1.3} & \tgpm{22.2}{1.4}
            & \tgpm{53.3}{0.8} & \tgpm{59.6}{1.9}
            & \textcolor{gray}{52.1} & \textcolor{gray}{--} \\
            & \textaccharmonic{}
            & \tupm{78.4}{0.8} & \tpm{20.9}{0.5}
            & \tbpm{52.5}{0.4} & \tupm{68.9}{0.8}
            & 55.2 & \textbf{4} \\
        \bottomrule
    \end{tabular}}
    \cvspace{-4pt}
\end{table}

